Optimal Data Acquisition for Statistical Estimation

We consider a data analyst's problem of purchasing data from strategic agents to compute an unbiased estimate of a statistic of interest. Agents incur private costs to reveal their data and the costs can be arbitrarily correlated with their data. Once revealed, data are verifiable. This paper focuses on linear unbiased estimators. We design an individually rational and incentive compatible mechanism that optimizes the worst-case mean-squared error of the estimation, where the worst-case is over the unknown correlation between costs and data, subject to a budget constraint in expectation. We characterize the form of the optimal mechanism in closed-form. We further extend our results to acquiring data for estimating a parameter in regression analysis, where private costs can correlate with the values of the dependent variable but not with the values of the independent variables.

==> summary-extensions.tex <==
%We show how to extend our approach in multiple directions, deferred to the appendix. In this section, we briefly describe our extensions.

\paragraph{Multi-dimensional moment estimation:} We show in Appendix~\ref{sec:multidimensional-linear} that we can in fact extend our analysis to the case where $m(z)$ is a $d$-dimensional vector with support $[0,1]^d$ and we are trying to estimate each coordinate of $\E\left[m(z)\right]$ so as to minimize the mean-squared error of the estimator. More precisely, we prove---under the condition that all of the corners of the hypercube $[0,1]^d$ are contained in the support of $m(z)$---that the $d$-dimensional problem reduces exactly to solving the $1$-dimensional problem discussed in Section~\ref{sec:moment-estimation}. One can therefore use the results of Section~\ref{sec:moment-estimation} to design an optimal allocation rule under the budget constraint in the multi-dimensional setting.

\paragraph{Linear regression:} We extend our results beyond moment estimation, to a multi-dimensional linear regression task. In this setting, an agent's information consists of a feature vector $x_i \in \reals$, an outcome value $y_i \in \reals$, and a residual value $\epsilon_i \in \reals$, drawn in the following manner: first, $x_i$ is drawn from an unknown distribution $\cX$.  Then, independently from $x_i$, the pair $(c_i, \epsilon_i)$ is drawn from a joint distribution $\cD$ over $\reals^2$.  The marginal distribution over costs, $\cD_c$, is known to the designer, but not the full joint distribution $\cD$.  Then $y_i$ is defined to be 
$$y_i = x_i^\top \theta^* + \epsilon_i,$$ 
where $\theta^* \in \Theta$ with $\Theta$ a compact subset of $\reals^d$. We assume the marginal distribution over $\epsilon_i$ is supported on some bounded range $[L,U]$ and has expected value $0$.  (So, in particular, $L \leq 0 \leq U$.)  

When a survey mechanism buys data from agent $i$, the pair $(x_i, y_i)$ is revealed. However, the value of $\epsilon_i$ is not revealed to the survey mechanism.  The goal of the designer is to estimate the parameter vector $\theta^*$. The analyst wants to design a survey mechanism to buy from the agents, then compute an estimate of $\theta$, while not paying each agent more than the total budget $\bar{B}$ per agent in expectation. 

One can interpret $x_i$ as a vector of publicly-verifiable information about agent $i$, which might influence a (possibly sensitive) outcome $y_i$.  For example, $x_i$ might consist of demographic information, and $y_i$ might indicate the severity of a medical condition.  The coefficient vector $\theta^*$ describes the average effect of each feature on the outcome, over the entire population.  Under this interpretation, $\epsilon_i$ is the residual agent-specific component of the outcome, beyond what can be accounted for by the agent's features.  We can interpret the independence of $x_i$ from $(c_i, \epsilon_i)$ as meaning that each agent's cost to reveal information is potentially correlated with their (private) residual data, but is independent of the agent's features.  

As in Section~\ref{sec:moment-estimation}, the analyst wants to design a survey mechanism to buy from the agents,  obtain data from the set $S$ of elicited agents, then compute an estimate $\hat{\theta}_S$ of $\theta$, while not paying each agent more than the total budget $\bar{B}$ per agent in expectation.  To this end, the analyst designs an allocation rule $A$ and a pricing rule $P$ so as to minimize the $\sqrt{n}$-normalized worst-case asymptotic mean-squared error of $\hat{\theta}_S$ as the population size goes to infinity. Our mechanism will essentially be optimizing the coefficient in front of the leading $1/n$ term in the mean squared error, ignoring potential finite sample deviations that decay at a faster rate than $1/n$. Note that we will design allocation and pricing rules to be independent of the population size $n$; hence, the analyst can use the designed mechanism even if the exact population size in unknown.

The analyst's estimate is given by the value $\hat{\theta}_S$ that minimizes the Horvitz-Thompson mean-squared error $\E[(y_i-x_i^\top \theta^*)^2]$, i.e.,
\begin{equation}
 \hat{\theta}_S = \argmin_{\theta \in \Theta} \sum_i  \frac{1 \{i \in S\}}{A(c_i)} (y_i-x_i^\top \theta)^2.
\end{equation}
Further, we make the following assumption on the distribution of data points:
\begin{assumption}[Assumption on the distribution of features]\label{as: x-distribution}
$E[x_i x_i^\top]$ is finite and positive-definite, and hence invertible.
\end{assumption}
Finite expectation is a property one may expect real data such has age, height, weight, etc. to exhibit. The second part of the assumption is satisfied by common classes of distributions, such as multivariate normals. 

We now state our main results, and defer proofs and technical details to Appendix~\ref{sec:linear-regression}. We first show that our estimator is consistent, i.e. it converges in probability towards the true parameter $\theta^*$ as the population size grows to infinity:
\begin{lemma}
Under Assumption~\ref{as: x-distribution}, for any allocation rule $A > 0$ that does not depend on $n$, $\hat{\theta}_S$ is a consistent estimator of $\theta^*$.
\end{lemma}

As in Section~\ref{sec:moment-estimation}, we now assume costs are drawn from a discrete set, say $\cC = \{c_1, \ldots, c_{\ubc} \}$.  We will then write $A_t$ for an allocation rule conditional on the cost being $c_t$, and $\pi_t$ the probability of the cost of an agent being $c_t$.  We will further assume that $\bar{B} < \sum_{t=1}^{\ubc} \pi_t c_t$, meaning that it is not feasible to accept all data points, since otherwise it is trivially optimal to set $A_t = 1$ for all $t$. Our main result, that characterizes the form of the optimal allocation rule, is then given by:
\begin{theorem}
Under the assumptions described above, if $U^2 \geq L^2$, an optimal allocation rule $A$ has the form
\begin{enumerate}
\item $A_t = \min\left(1,\alpha \frac{|L|}{\sqrt{c_t}}\right)$ for $t < t^-$
\item $A_t = \bar{A}$ for all $t \in \{ t^-, \ldots, t^+\}$
\item $A_t = \min\left(1,\alpha \frac{U}{\sqrt{c_t}}\right)$ for $t > t^+$
\end{enumerate}
for $\bar{A}$ and $\alpha$ positive constants that do not depend on $n$, and $t^-$ and $t^+$ integers with $t^- \leq t^+$.
\end{theorem}
When $L^2 \geq U^2$, the form of the allocation rule can be obtained by reversing the roles of $L$ and $U$ (for more details, see Appendix~\ref{sec:linear-regression}). We remark that the solution for the linear regression case exhibits a structure that is similar to the structure of the optimal allocation rule for moment estimation (see Theorem~\ref{thm:main-moment-estimation}): it exhibits a pooling region in which all cost types are treated the same way, and changes in the inverse of the square root of the cost outside said pooling region. However, we note that we may now choose to pool agents together in an intermediate range of costs, instead of pooling together agents whose costs are below a given threshold. 

\paragraph{Non-linear regression:} We further show that our results extend to non-linear regression, i.e. when $y_i$ is generated by a process of the more general form 
$$y_i = f(\theta^*,x_i) + \epsilon_i,$$
 under a few additional assumptions on the distribution of $x$ and on the regression function $f$. Said assumptions are discussed in more detail in Appendix~\ref{app:nonlinear-regression}.
 
%\blcomment{Is it possible to include a theorem statement that elaborates on the ``mild assumptions''?}\jzcomment{There are a few of them and it's probably going to take up some space. I'm thinking those are mild but maybe you want to check the appendix to see if you agree on what I call "mild"}

%\paragraph{The case of many populations:} We generalize the setting of Section~\ref{sec:moment-estimation} to the case of several populations with possibly different population sizes and distributions of costs.  The data analyst wants to buy data from agents from each population, and estimate a parameter or expected moment $\theta_p = \E[m_p(z)]$ of each population $p$, where $m_p:\cZ_p\rightarrow [0,1]$ is a moment function that can take values both $0$ and $1$ for some $z_p$. The analyst must do so without spending more than his allocated budget $B$ in expectation. To this effect, the analyst first decides how to split his total budget $B$ between different populations. The analyst then picks an allocation rule, a payment rule  and a linear unbiased estimatorof $\theta_p$ that is a function of the elicited sample $S_p$ in population $p$ and potentially the distribution of costs $\cF_p$ and the allocation rule. The analyst's goal is to minimize a weighted sum of the worst-case variances of the estimators. We give an efficient algorithm to optimally split the total budget $B$ between the many different populations in Section~\ref{sec:many-populations}.
%\jzcomment{Delete this last paragraph if we don't add the many population case}




